Feature Representation Learning for Click-through Rate Prediction: A Review and New Perspectives

Representation learning has been a critical topic in machine learning. In Click-through Rate Prediction, most features are represented as embedding vectors and learned simultaneously with other parameters in the model. With the development of CTR models, feature representation learning has become a trending topic and has been extensively studied by both industrial and academic researchers in recent years. This survey aims at summarizing the feature representation learning in a broader picture and pave the way for future research. To achieve such a goal, we first present a taxonomy of current research methods on feature representation learning following two main issues: (i) which feature to represent and (ii) how to represent these features. Then we give a detailed description of each method regarding these two issues. Finally, the review concludes with a discussion on the future directions of this field.

==> old/method_old.tex <==

\section{Tables}


\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|ccc}
        \hline
        Methods & Goal & Granularity & Method \\
        \hline
        LPFS & Feature & Field & Pruning \\
        AutoField & Feature & Field & AutoML \\
        AdaFS & Feature & Sample & AutoML \\
        \hline
        AutoDis & Feature & Feature & Soft Discretization \\
        CE & Feature & Feature & Product Quantization \\
        DHE & Feature & Feature & MLP \\
        \hline
        ESAPN & Embed & - & -   \\
        NIS & Embed & - & -     \\
        DNIS & Embed & - & -    \\
        AutoEmb & Embed & - & - \\
        AutoDim & Embed & - & - \\
        RULE & Embed & - & -    \\
        DLRM & Embed & - & -    \\
        HAM & Embed & - & -     \\
        EMDE & Embed & - & -    \\
        MDE & Embed & - & -     \\
        Autosrh & Embed & - & - \\
        \hline
        PEP & Both & - & -\\
        OptEmbed & Both & - & -\\
        AutoGroup & Both & - & -\\
        iRazor & Both & - & -\\
        \hline
        AutoFIS & F.I. & - & -\\
        AutoFeature & F.I. & - & -\\
        AutoIAS & F.I. & - & -\\
        XCrossNet & F.I. & - & -\\
        AIM & F.I. & - & -\\
        AutoPI & F.I. & - & -\\
        NAS-CTR & F.I. & - & -\\
        FIGAT & F.I. & - & -\\
        L0-SIGN & F.I. & - & -\\
        HIRS & F.I. & - & -\\
        FIVES & F.I. & - & -\\
        PROFIT & F.I. & - & -\\
        SAFM & F.I. & - & - \\
        OptInter & F.I. & - & - \\
        GLIDER & F.I. & - & - \\
        \hline
    \end{tabular}
    }
    \caption{Latex default table}
    \label{tab:plain1}
\end{table}


% \begin{table*}
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c|l|ccc|ccc|ccc}
%         \hline
%         & \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{Feature Selection} & \multicolumn{3}{c|}{Embedding Selection} & \multicolumn{3}{c}{Feature Interaction Selection} \\
%         \cline{3-11}
%         & & Adopted & Granularity & Method & Adopted & Granularity & Method & Adopted & Granularity & Method \\
%         \hline
%         \multirow{3}{*}{FS}
%         & LPFS~\shortcite{FS-LPFS} & \Checkmark & Field & Pruning & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         & AutoField~\shortcite{FS-AutoField} & \Checkmark & Field & Gumbel-softmax & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         & AdaFS~\shortcite{FS-AdaFS} & \Checkmark & Sample & Gumbel-softmax & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         \hline
%         \multirow{3}{*}{FH}
%         & AutoDis~\shortcite{FH-AutoDis} & \Checkmark & Feature & - & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         & CE~\shortcite{FH-CE} & \Checkmark & Feature & Product Quantization & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         & DHE~\shortcite{FH-DHE} & \Checkmark & Feature & MLP & \XSolidBrush & - & - & \XSolidBrush & - & - \\
%         \hline
%         \multirow{11}{*}{EDS}
%         & ESAPN~\shortcite{ES-ESAPN} & \XSolidBrush & - & - & \Checkmark & Predefined Mask & RL & \XSolidBrush & - & - \\
%         & NIS~\shortcite{ES-NIS} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & DNIS~\shortcite{ES-DNIS} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & AutoEmb~\shortcite{ES-AutoEmb} & \XSolidBrush & - & - & \Checkmark & Predefined Mask & Gradient-based AutoML & \XSolidBrush & - & - \\
%         & AutoDim~\shortcite{ES-AutoDim} & \XSolidBrush & - & - & \Checkmark & Predefined Mask & Gradient-based AutoML & \XSolidBrush & - & - \\
%         & RULE~\shortcite{ES-RULE} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & DLRM~\shortcite{ES-DLRM} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & HAM~\shortcite{ES-HAM} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & EMDE~\shortcite{ES-EMDE} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & MDE~\shortcite{ES-MDE} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         & Autosrh~\shortcite{ES-Autosrh} & \XSolidBrush & - & - & \Checkmark & - & - & \XSolidBrush & - & - \\
%         \hline
%         \multirow{15}{*}{FIS}
%         & AutoFIS~\shortcite{FIS-AutoFIS} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & high-order & GRDA Pruner \\
%         & AutoFeature~\shortcite{FIS-AutoFeature} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & 2nd-order & Evolutional Search \\
%         & AutoGroup~\shortcite{FIS-AutoGroup} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & high-order & AutoML \\
%         & XCrossNet~\shortcite{FIS-XCrossNet} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & - & - \\
%         & AutoPI~\shortcite{FIS-AutoPI} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & 2nd-order & AutoML \\
%         & NAS-CTR~\shortcite{FIS-NAS-CTR} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & - & - \\
%         & FIGAT~\shortcite{FIS-FIGAT} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & - & - \\
%         & L0-SIGN~\shortcite{FIS-L0-SIGN} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & 2nd-order & GNN edge search \\
%         & HIRS~\shortcite{FIS-HIRS} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & high-order & GNN edge search \\
%         & FIVES~\shortcite{FIS-FIVES} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & high-order & GNN edge search \\
%         & PROFIT~\shortcite{FIS-PROFIT} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & high-order & Progressive search \\
%         & SAFM~\shortcite{FIS-SAFM} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & - & - \\
%         & OptInter~\shortcite{FIS-OptInter} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & 2nd-order & AutoML \\
%         & GLIDER~\shortcite{FIS-GLIDER} & \XSolidBrush & - & - & \XSolidBrush & - & - & \Checkmark & - & - \\
%         \hline
%         \multirow{4}{*}{FS \& EDS}
%         & PEP~\shortcite{FS+ES-PEP} & \Checkmark & Feature & Pruning & \Checkmark & Element & Pruning & \XSolidBrush & - & - \\
%         & OptEmbed~\shortcite{FS+ES-OptEmbed} & \Checkmark & Feature & Pruning & \Checkmark & Continuous Elements & Evolutional Search & \XSolidBrush & - & - \\
%         & iRazor~\shortcite{FS+ES-iRazor} & \Checkmark & Field & Gradient-based AutoML & \Checkmark & Predefined Masks & Gradient-based AutoML & \XSolidBrush & - & - \\
%         \hline
%         \multirow{1}{*}{FIS \& EDS}
%         & AIM~\shortcite{FIS+ES-AIM} & \XSolidBrush & - & - & \Checkmark & - & - & \Checkmark & - & - \\
%         & AutoIAS~\shortcite{FIS+ES-AutoIAS} & \XSolidBrush & - & - & \Checkmark & - & - & \Checkmark & - & - \\
%         \hline
%     \end{tabular}
%     }
%     \caption{Latex default table}
%     \label{tab:plain}
% \end{table*}




% \begin{table*}[!htbp]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         Order & Granularity & Methods & Papers \\
%         \hline
%         % 1st & field & shallow & \\
%         1st & field & bi-lvl & AutoField~\shortcite{FS-AutoField} \\
%         1st & field & pruning & LPFS~\shortcite{FS-LPFS} \\
%         1st & sample & bi-lvl & AdaFS~\shortcite{FS-AdaFS} \\
%         % 1st & feature & pruning & \\
%         \hline
%         2nd & field & bi-lvl & OptInter~\shortcite{FIS-OptInter}\\
%         3nd & field & GNN & L0-SIGN~\shortcite{FIS-L0-SIGN} \\
%         \hline
%         higher & field & bi-lvl & AutoFIS~\shortcite{FIS-AutoFIS},  AutoPI~\shortcite{FIS-AutoPI}, PROFIT~\shortcite{FIS-PROFIT} \\
%         higher & field & e.s. & AutoFeature~\shortcite{FIS-AutoFeature} \\
%         higher & field & GNN & HIRS~\shortcite{FIS-HIRS}, FIVES~\shortcite{FIS-FIVES} \\
%         \hline
%     \end{tabular}
%     \caption{Taxonomy of the representation learning}
%     \label{tab:taxonomy}
% \end{table*}











